Technical Debts and Faults in Open-source Quantum Software Systems: An Empirical Study

Quantum computing is a rapidly growing field attracting the interest of both researchers and software developers. Supported by its numerous open-source tools, developers can now build, test, or run their quantum algorithms. Although the maintenance practices for traditional software systems have been extensively studied, the maintenance of quantum software is still a new field of study but a critical part to ensure the quality of a whole quantum computing system. In this work, we set out to investigate the distribution and evolution of technical debts in quantum software and their relationship with fault occurrences. Understanding these problems could guide future quantum development and provide maintenance recommendations for the key areas where quantum software developers and researchers should pay more attention. In this paper, we empirically studied 118 open-source quantum projects, which were selected from GitHub. The projects are categorized into 10 categories. We found that the studied quantum software suffers from the issues of code convention violation, error-handling, and code design. We also observed a statistically significant correlation between code design, redundant code or code convention, and the occurrences of faults in quantum software.

==> image/charts/combine_fig_table.tex <==

\begin{table}[ht!]

	\begin{minipage}{0.9\linewidth}
		\centering
		
		\includegraphics[width=1.0\textwidth]{image/boxplot_files.pdf}
		
		\captionof{figure}{Percentage of unique files contributing to 80\% of the overall technical debts across the snapshots of the selected projects}
		\label{figu:box-unique-files}
	\end{minipage}
\end{table}

==> image/charts/commits_distrib.tex <==


 \begin{figure}

\centering
%        \begin{subfigure}[b]{0.65\textwidth}
%                \includegraphics[width=\linewidth]{image/plot_0.pdf}
                %\caption{Ass(qubiter)}
                %\label{fig:sub-assembly1}
%        \end{subfigure}%

        %%% row2
        \hfill
        
%         \begin{subfigure}[b]{0.65\textwidth}
%                \includegraphics[width=\linewidth]{image/plot_1.pdf}
                %\caption{Exp(PyQLab)}
                %\label{fig:sub-Experimentation1}
%        \end{subfigure}%
        
        \caption{The distribution of commits across different day frames\mehdi{time frames?} for the $6$ categories of quantum projects. The y-axis indicates the number of commits, and the x-axis indicates the day frames\mehdi{number of days} from 30 to 180 days with the interval of 30 days.}\label{fig:commits-dirstribution}
\end{figure}

==> image/charts/plot_commits.tex <==

\begin{figure}
\centering
%\scalebox{0.75}{
\begin{tikzpicture}[x={(0.0025,0)}, scale=0.35]
\foreach  \l/\x/\c[count=\y] in {
Orbital Energies/8445.1/definedGray,
Configuration Interaction/4769.8/definedGray,
Path Integral/4551/definedGray,
Arrays and Matrix Operations/4333.9/definedGray,
Gates Decomposition/4257.5/definedGray,
Parameter Checks and Selection/4168.3/definedGray,
Message Passing/4132.8/definedGray,
Memory and Performance Optimization/4072.3/definedGray,
Programming Pulse/4054.1/definedGray,
Code Integration/3972.5/definedGray,
Feature Expansion/3442.2/definedGray,
I\/O and Text Format/3379.6/definedGray,
Program Optimization/3283.3/definedGray,
Test Implementation/3224.1/definedGray,
Code Refactoring/3116.6/definedGray,
Data Structures and Operations/3022.1/definedGray,
Compiler Optimization/2882.5/definedGray,
Module Testing/2824.7/definedGray,
Configuration Files/2804.9/definedGray,
Comments\/ Doc-string/2661.4/definedGray,
Dependency Management/2659.7/definedGray,
Continuous Integration/2572.7/definedGray,
Circuit Design/2469.4/definedGray,
Legacy Code \& Deprecation/1019.6/definedGray}
{\node[left] at (0,\y) {\l};
\fill[\c] (0,\y-.3) rectangle (\x,\y+.3);
\node[right] at (\x, \y) {\x};}
\draw (0,0) -- (8000,0);
\foreach \x in {2000,4000,...,8000}
{\draw (\x,.02) -- (\x,0) node[below] {\x};}
\draw (0,0) -- (0,0.15);
\end{tikzpicture}
%}

\caption{The median of average time (in hours) between the dates of bugs inducing and bugs fixing commits.
}
\label{fig:topicQuestions}
\vspace{-12pt}

\end{figure}
	

==> subsections/04-RQ4.tex <==
%\Le{General comment: I see both fault and bug are used in this subsection (e.g., fault in the first paragraph, bug in Table 7). I changed all faults to bugs in RQ3, but I see that you may prefer faults. So I leave this work to you to make all the terms consistently. Please also check everywhere in the paper about the terms, we should make all consistently.}
\subsection{\textbf{RQ4: What Are the Characteristics of the Changes That Introduced Quantum Software Faults?}}
\label{sec:result-bugs-introduced}

\MO{Reviewer1: -How do you identify high-level topics from low-level ones? Moreover, I would suggest presenting your results for RQ4 by looking at high-level topics. Now, it is unclear how you chose the topics to be investigated more in depth. Each category has to be described and for some of them examples may help in better understanding the activity inducing the faults.
-Actually RQ4 seems to be unrelated to the other three RQs and is not complete in terms of presentation. You can think about spending more time in refining the previous three RQs and maybe drop the last one from the current version of the paper.
-The examples being reported for RQ4 need to be accompanied by the commit message since it is used for clustering and determining the topic. Moreover, it would be interesting to see how the fault inducing commit is related to the fault fixing commit and how both of them deal with TDs.
-The examples reported in Data Structure & Operations seem more related to compatibility issues. The same occurs for the example in the Configuration Files topic where the last one seems to relate to Continuous Integration. Probably it is required to manually validate the performance of LDA in clustering the commit messages.}

\MO{Reviewer2: - In section 5.4, the discussion around topics, I was eagerly looking for more non-traditional topics like "Chemical Calculation" but I got disappointed as they were not discussed.}

This section discusses the characteristics of the fault-inducing commits.
We present the faults-inducing activities as topics generated using topic modelling technique described in Section \ref{sec:model-labels}. We will use the information of fault-inducing and fault-fixing commits to illustrate the dominating topics and how long it took before the faults got fixed.



\begin{table}[t]
     \caption{Topics extracted from the messages of fault-inducing commits, along with the the category of the topics and the percentage of coverage of the repositories (\% coverage) by the corresponding topics.}
     \label{tab:topics}
     \begin{adjustbox}{width=0.75\textwidth,center}
         \begin{tabular}{l |l l  r}\toprule
        \rowcolor{gray!20}
         \textbf{} & \textbf{Low level topic} &\textbf{High level topic} & \multicolumn{1}{c}{\textbf{\% coverage}} \\ \midrule
    
        1&Compiler Optimization&Optimization & 75\% \\ %hline, measurement, simulator, statement\\ %hline, process, work, simple, implement, measure, code, logic\\ %hline
        \rowcolor{gray!15}
        2&I/O \& Text Format&File Management & 70\% \\ %hline, replace, image, expression\\ %hline, find, produce, show, range, testing, clear\\ %hline
        3&Calibration \& Visualization&Programming & 69\%\\ %hline, car, merge, schedule, function\\ %hline, condition, convert, comment, embed, base\\ %hline
        \rowcolor{gray!15}
        4&Program Optimization& Optimization & 69\%\\ %hline, device, check, case\\ %hline, coverage, buffer, testing, cleanup, single, comment\\ %hline
        5&Feature Expansion&Implementation & 69\%\\ %hline, provide, part, specific, model\\ %hline, exist, easy, constant, optional, feature, include\\ %hline
        \rowcolor{gray!15}
        6&Code Refactoring&Refactoring & 69\%\\ %hline, functionality, util, refactor\\ %hline, base, constructor, todo, type_hint, definition, copyright, refactore\\ %hline
        7&Data Structure \& Operations&Programming& 71\% \\ %hline, key\\ %hline, handle, backend, base\\ %hline, replace, dict, status, converter, qobj\\ %hline
        \rowcolor{gray!15}
        8&Legacy Code/Deprecation&Refactoring/Rewrite & 71\%\\ %hline, address, begin, bug\\ %hline, deprecation, namespace, clean, conversion, split, late\\ %hline
        %\rowcolor{gray!10}
        %9&Documentation&Documentation&change, documentation, format, reference, link, section, miss, tutorial, note, readme, description, fix & \\ %hline, page, table, text, include\\ %hline, manual, figure, final, edit, main\\ %hline
        9&Chemical Calculation&Molecular mechanics& 61\%\\ %hline, charge, cell, density\\ %hline, restart, scf, core, moment, computation\\ %hline
        \rowcolor{gray!15}
        10&Memory \& Performance Optimization&Optimization & 69\%\\ %hline, time, common, kernel, large, request\\ %hline, wavefunction, speed, problem, cc_cdfa, additional\\ %hline
        11&Code Integration&Release Engineering & 70\%\\ %hline, header, command, check, internal, simplify\\ %hline, complete, avoid, part, include\\ %hline
        \rowcolor{gray!15}
        12&Arrays \& Matrix Operation& & 68\%\\ %hline, due, double, miss, constructor\\ %hline, return, correct, conversion, simple, reference\\ %hline
        13&Gates Decomposition&Algorithm/Optimization& 70\% \\ %hline, direct, setup, view, factor, addition\\ %hline
        \rowcolor{gray!15}
        14&Configuration Files&Scripting/Environment& 70\%\\ %hline, component, color, setting, seed, directory\\ %hline, multiple, button, step, enable\\ %hline
        15&Configuration Interaction& & 65\%\\ %hline, single, find, large, sign\\ %hline, select, weight, determinant, previous, column\\ %hline
        \rowcolor{gray!15}
        16&Module Updates&& 69\%\\ %hline, issue, fit, solve\\ %hline, improvement, clean, stuff, part, filter\\ %hline
        17&Continuous Integration&Release Engineering& 69\%\\ %hline, user, window, cache, build, ensure\\ %hline, tag, commit_add, failure, script, part\\ %hline
        %\rowcolor{gray!10}
        %19&Comments/docstring&Documentation&add, fix, test, update, docstre, docstring, change, remove, code\_review & \\ %hline, apply\_suggestion, template, import, make, comment, sample\\ %hline, wire, linte, minor, black, rename\\ %hline
        \rowcolor{gray!15}
        18&Circuit Design&Programming& 67\%\\ %hline, label, control, deprecate\\ %hline, draw, remove, visualization, op, mergify\\ %hline
        19&Dependency Management&Release Engineering& 73\% \\ %hline, target, instal, compile, project, library\\ %hline, compiler, installation, tool, external, late\\ %hline
        \rowcolor{gray!15}
        20&Messages Passing&Concurrency & 66\% \\%hline, distribute\\ %hline, object, basis_set, cdfa, network, share\\ %hline
        21&Parameter Checks \& Selection&Optimization& 69\%\\ %hline, save, branch\_extra, branch\_prerelease, cba\\ %hline, address, implement, unused, scale, properly, apply\\
        %hline
        \rowcolor{gray!15}
        22&Path Integral&Quantum Mechanics& 69\% \\ %hline, storage\\ %hline, convention, contraction, related, contribution, product, calculate\\ %hline
        				
        \bottomrule
        \end{tabular}  
     \end{adjustbox}
\end{table}

%\Le{Where is this footnote?\Mehdi{I think it was assigned to the table}}
%\footnotetext{\url{https://github.com/openjamoses/emse-quantum/blob/main/Quantum-topics.csv}}


Table \ref{tab:topics} shows the different topics found from the changes that introduced faults.
%describing the activities that introduce faults during the development of quantum software systems extracted from fault-inducing commit message using topic mode technique.  %The highlighted columns indicate the topics that were merged together due to their semantic similarity. 
Using these categories, we further classified the topics into different groups, indicating the root causes of the faults. The column `\% coverage' in Table \ref{tab:topics} indicates the percentage of unique projects where the messages of fault-inducing commits contributed to a topic.


We found a total of 22 topics from the fault-inducing commits. We presented the fault-inducing topics both at higher and lower level of granularity. For example,  topics  `Code Integration', `Chemical calculation', and 'Code Refactoring' are coarse-grained whereas topics `Data Structure \& Operations', `Message Passing', `Circuit design', `Module Updates' are fine-grained. These topics are further broken down into higher-level topics representing each topic's categories such as Optimization, File Management, Programming, Refactoring, Release Engineering and Quantum mechanics. In the following paragraphs, we will discuss some of the topics by referring to the corresponding commit messages to understand the factors that may introduce faults in quantum software.


\nd \textbf{Compiler Optimization:} This topic is about faults introduced when implementing and fixing the problems with the compilation of quantum programs to allow for fewer resources and faster execution during program transformation to a subsequent machine-readable program. 

One fault-inducing change related to this topic is the commit
\href{https://github.com/BBN-Q/pyqgl2/commit/938e1fa75b790771829e5c1ab12fd4beee3e6bb9}{\texttt{\#938e1fa75}} in \texttt{BBN-Q/pyqgl2} (a quantum programming language and compiler),
% \hashid{\texttt{\#938e1fa75}}\footnote{\url{https://github.com/BBN-Q/pyqgl2/commit/938e1fa75b790771829e5c1ab12fd4beee3e6bb9}}, 
which attempted to fix a problem related to meta-programming. This commit added a new file with over $60$ lines of code (code changes to track the local symbol values during function calls to convert the call to the function, instead of an application of the local variable). According to the in-code comments in this commit, a similar problem was previously solved for the method stub and extending the similar implementation to other methods other than the stubs. 
%However, according to our analysis, this change was detected as fault-inducing that was later fixed by a commit with
%\href{https://github.com/BBN-Q/pyqgl2/commit/38edd331d90d55c723fd4cd098dbb42932b1f402}{\hashid{\texttt{\#38edd33}}}
% \hashid{\#38edd33}\footnote{\url{https://github.com/BBN-Q/pyqgl2/commit/38edd331d90d55c723fd4cd098dbb42932b1f402}}. 

Another commit that introduced faults of this category is a refactoring and fault-fixing commit 
% \hashid{\texttt{\#7c68527}}\footnote{\url{https://github.com/Qiskit/qiskit-terra/commit/7c68527d585b4547c49f16c4a8748ea52416713e}}, 
\href{https://github.com/Qiskit/qiskit-terra/commit/7c68527d585b4547c49f16c4a8748ea52416713e}{{\texttt{\#7c68527}}} in \path{Qiskit},
which modified the backend of the framework~\cite{qiskit:backends}
% \footnote{\url{https://medium.com/qiskit/qiskit-backends-what-they-are-and-how-to-work-with-them-fb66b3bd0463}} 
for the quantum project \texttt{Qiskit/qiskit-terra}. The commit modified $40$ different files with over $759$ added lines and $242$ deleted lines with the changes such as re-introduction of the ability to pass an open circuit and unify the backend's handling configurations, and refactored of a wrapper function to accept the backend as string instead of
the object. This commit induced faults that were fixed by 48 other commits and more than 15 developers. 
%Some of the fault-fixing commits include
% \#d05f7b8\footnote{\url{https://github.com/Qiskit/qiskit-terra/commit/d05f7b82298275f450871150cea47f48170b8f1d}}, 
%\href{https://github.com/Qiskit/qiskit-terra/commit/d05f7b82298275f450871150cea47f48170b8f1d}{\hashid{\texttt{\#d05f7b8}}},
% \#08607e2 \footnote{\url{https://github.com/Qiskit/qiskit-terra/commit/08607e2153bc811fbd80beb93370e31e06507dc6}},
%\href{https://github.com/Qiskit/qiskit-terra/commit/08607e2153bc811fbd80beb93370e31e06507dc6}{\hashid{\texttt{\#08607e2}}},
% \#5a1b38b\footnote{\url{https://github.com/Qiskit/qiskit-terra/commit/5a1b38ba9afe6914871c647a9cb3eea65cce97d1}}, 
%\href{https://github.com/Qiskit/qiskit-terra/commit/5a1b38ba9afe6914871c647a9cb3eea65cce97d1}{\hashid{\texttt{\#5a1b38b}}},
% \#182c2ee \footnote{\url{https://github.com/Qiskit/qiskit-terra/commit/182c2eefdf4a6b614793ac55eeb197bf015be7f6}}, 
%\href{https://github.com/Qiskit/qiskit-terra/commit/182c2eefdf4a6b614793ac55eeb197bf015be7f6}{\hashid{\texttt{\#182c2ee}}},
%and 
% \#cac7c6a \footnote{\url{https://github.com/Qiskit/qiskit-terra/commit/cac7c6a2631d76ef3e811a5c943a2b9101fed240}}, 
%\href{https://github.com/Qiskit/qiskit-terra/commit/cac7c6a2631d76ef3e811a5c943a2b9101fed240}{\hashid{\texttt{\#cac7c6a}}},
%that was later identified to modify the similar lines of codes in the files changed by the fault-inducing commit \hashid{\texttt{\#7c68527}}.

\nd \textbf{Data Structure \& Operations:} This topic relates to the management and operations performed on large amounts of data, such as organizing and formatting the data for storage or creating a model from the data. For example, the commit 
%Example of changes that introduce faults related to \textit{Data Structure \& Operations} is a commit with 
% \hashid{\#c65b6da}\footnote{\url{https://github.com/ericchansen/q2mm/commit/c65b6da14f26f5a3be176a93ff11178975692b9e}} 
\href{https://github.com/ericchansen/q2mm/commit/c65b6da14f26f5a3be176a93ff11178975692b9e}{{\texttt{\#c65b6da}}}
in the project \texttt{ericchansen/q2mm} (q2mm stands for `quantum mechanics to molecular mechanics', which is used for optimizing force field). This commit refactored up to $12$ files, adding $266$ new lines of code and removing $414$ lines of code. The changes are mainly related to the datatype choices to be compatible with Python2/Python3 and to improve the coding styles. The changes include the use from iterator to lists, changing the data structure \path{map} to \path{list}, and replacing \path{dict.iter*()} by \path{dict.*()}.
This refactoring commit %detected as fault-inducing because similar lines in files changed during refactoring 
was later fixed by 2 other commits.%, among the commits including reverting back some of the changes \hashid{\#fb7d379}\footnote{\url{https://github.com/ericchansen/q2mm/commit/fb7d379565e266b59e25746ff84f53454e15f811}} and performing fault-fixes to the similar lines of code \hashid{\#e4dbda6}\footnote{\url{https://github.com/ericchansen/q2mm/commit/e4dbda64bbb8aa8fb0df262e0b1d42b53aabc3f0}}.  

Another example is in the quantum Assembly project \texttt{lanl/qmasm} (a quantum macro assembler for D-Wave systems to control hardware and as compilers to implement higher-level languages). The commit 
% \hashid{\#88e2aa3}\footnote{\url{https://github.com/lanl/qmasm/commit/88e2aa3275fe2d7c56beec04afaa63d1affa5469}} 
\href{https://github.com/lanl/qmasm/commit/88e2aa3275fe2d7c56beec04afaa63d1affa5469}{{\texttt{\#88e2aa3}}}
is associated with $6$ changed files that removed the unnecessary conversions of Python \path{list} datatype, which was mainly used in the iterator context. 
We observed that the changes in the commit related to modifying the data structures and operations such as sorting, dictionary/list iteration were fixed by 10 later commits.
%However, according to our analysis, these changes related to modifying the data structures/operations such as sorting, dictionary/list iteration induced more faults in the software that were later modified by more-than $10$ fault-fixing commits.% Among the fault-fixing changes include variables correction\hashid{\#c62315}\footnote{\url{https://github.com/lanl/qmasm/commit/c623159aafd8670f2e7ad91ec9ad9aa9a3f70392}},  Our analysis indicates that commits inducing bugs in this category cover about $73\% (95)$ of the studied quantum projects.


\nd \textbf{Memory \& Performance Optimization:} This topic is about the changes for quantum program's performance, memory leakage, and improvement of usability. The topic indicates that developers introduce faults during the process of optimizing memory usage and the quantum system's performance. An example is the commit
%of the modification that introduces faults is a commit with
% \hashid{\#c9798e6}\footnote{\url{https://github.com/qutip/qutip/commit/c9798e65a675b44ffb485d7da25370e9828c0716}} 
\href{https://github.com/qutip/qutip/commit/c9798e65a675b44ffb485d7da25370e9828c0716}{{\texttt{\#c9798e6}}} in the project \texttt{qutip/qutip} (a quantum toolbox for simulating the dynamics of quantum systems). This commit modified $4$ files with $187$ new lines implementing a generic method for dynamically controlling memory saving. Another, the commit
% \hashid{\#e547d2c}\footnote{\url{https://github.com/hande-qmc/hande/commit/e547d2c0698413f3b5ff8cc538a5932d2d175d29}} 
\href{https://github.com/hande-qmc/hande/commit/e547d2c0698413f3b5ff8cc538a5932d2d175d29}{{\texttt{\#e547d2c}}} in the project \texttt{hande-qmc/hande} (an open-source stochastic quantum chemistry) 
implemented memory allocation only when memory is required by a given block of Hamiltonian. % with the quantum project 
%\texttt{hande-qmc/hande} (an open source stochastic quantum chemistry).

\nd \textbf{Code Integration:} This high level topic is about the faults introduced in quantum software due to the integration of code changes from different development branches to the central branch (\emph{i.e.,} Git branching and merging). This topic is known to be a common challenge, even for traditional software systems, especially in large projects involving multiple teams and branching activities among others~\cite{modern-release-bram,Openja:2020}. 
%The example of fault-inducing commit related to this topic 
For example, commits 
% \hashid{\#3fe015b}\footnote{\url{https://github.com/Qiskit/qiskit-terra/commit/3fe015b5c9eec41c26ffeb0b1a23c25f9abef2d5}},
\href{https://github.com/Qiskit/qiskit-terra/commit/3fe015b5c9eec41c26ffeb0b1a23c25f9abef2d5}{{\texttt{\#3fe015b}}},
% \hashid{\#4b2ab63}\footnote{\url{https://github.com/Qiskit/qiskit-terra/commit/4b2ab63ca7d9dc4a6c741ed33adaa6208c53e41b}},
\href{https://github.com/Qiskit/qiskit-terra/commit/4b2ab63ca7d9dc4a6c741ed33adaa6208c53e41b}{{\texttt{\#4b2ab63}}}
% \usepackage{}\href{}{\hashid{\texttt{\#}}}
and 
% \hashid{\#8592c7b}\footnote{\url{https://github.com/Qiskit/qiskit-terra/commit/8592c7b7fc9b988e61b9527c69dfecb564b2f6f2}} 
\href{https://github.com/Qiskit/qiskit-terra/commit/8592c7b7fc9b988e61b9527c69dfecb564b2f6f2}{{\texttt{\#8592c7b}}}
modified the project \texttt{Qiskit/qiskit-terra} (a Python-based program for writing quantum circuits in Qiskit to help manage the constraints of real hardware). These commits introduced faults either at the point of code integration or when integrating the code changes from different development branches with faulty commits. Concretely, the commit \path{#3fe015b} integrated multiple code changes from two development branches into the master branch incorporating respective changes related to fault fixes, refactoring, and new implementations with $17$ different files, $576$ added lines, and $143$ removed lines. We also observed this kind of fault in other quantum projects, including
\href{https://github.com/rigetti/pyquil}{\texttt{rigetti/pyquil}},
\href{https://github.com/rigetti/pyquil}{{\texttt{rigetti/pyquil}}},
% \texttt{qojulia/QuantumOptics.jl}\footnote{\url{https://github.com/qojulia/QuantumOptics.jl}}, 
\href{https://github.com/qojulia/QuantumOptics.jl}{\texttt{qojulia/QuantumOptics.jl}},
% \texttt{BBN-Q/pyqgl2}\footnote{\url{https://github.com/BBN-Q/pyqgl2}}, 
\href{https://github.com/BBN-Q/pyqgl2}{\path{BBN-Q/pyqgl2}},
% \texttt{cp2k/cp2k}\footnote{\url{https://github.com/cp2k/cp2k}}
\href{https://github.com/cp2k/cp2k}{\path{cp2k/cp2k}}, and
%(a software package for quantum chemistry and solid state physics) and 
% \texttt{QuTech-Delft/qtt}\footnote{\url{https://github.com/QuTech-Delft/qtt}}.
\href{https://github.com/QuTech-Delft/qtt}{\path{QuTech-Delft/qtt}}.


\nd \textbf{Arrays \& Matrix Operation:} This topic involve commits that introduce faults in the quantum source code when applying different operations to arrays and matrix and other related linear algebraic functions to describe the quantum operations, such as the qubits' states at the specific point in time, \emph{e.g.,} the commit  
% \hashid{\#39edb2f}\footnote{\url{https://github.com/TRIQS/triqs/commit/39edb2f84611fc576748cddd11e3a47d3828c15e}} 
\href{https://github.com/TRIQS/triqs/commit/39edb2f84611fc576748cddd11e3a47d3828c15e}{{\texttt{\#39edb2f}}}
in the project \texttt{TRIQS/triqs} (a multi-language toolbox to allow researchers to interact with quantum systems). This commit performed both refactoring and a fault-fixing change where $69$ different files were modified. The change implemented tensor factorization and used mesh array in the constructor. %, among others. 

Another example of fault-inducing commit of this category is the commit
\href{https://github.com/qojulia/QuantumOptics.jl/commit/c95ac80b79f959912178639d2bf3ed537b570034}{\texttt{{\#c95ac80}}}
% \hashid{\#c95ac80}\footnote{\url{https://github.com/qojulia/QuantumOptics.jl/commit/c95ac80b79f959912178639d2bf3ed537b570034}}
in the project \texttt{qojulia/QuantumOptics.jl} (a quantum numerical toolkit for simulating different ranges of quantum systems based on the Julia programming language). The commit added 135 new lines of code in the project. It also modified the code that used array reshaping and slicing (lazy operator multiplication) by implementing a new function that used linear array directly as a way to optimize the performance of loops.

We also observed this kind of fault from other quantum projects, including \texttt{votca/xtp} (a library to calculate the electronic properties of organic materials) \texttt{TRIQS/triqs}, \texttt{qutip/qutip}, \texttt{rigetti/rpcq} (a remote procedure calls frameworks and message specification), and \texttt{cp2k/cp2k}.
%According to our analysis, other quantum projects of this category with the highest percentage of commits introducing faults include \texttt{votca/xtp} (a library to calculate the electronic properties of organic materials) \texttt{TRIQS/triqs}, \texttt{qutip/qutip}, \texttt{rigetti/rpcq} (a remote procedure calls frameworks and message specification), and \texttt{cp2k/cp2k}. %among others.
    
    
\nd \textbf{Configuration Files:} This topic is about faults introduced during the implementation or modification of the configuration related files containing different parameters and other associated settings used in quantum software.  
The commit 
% \hashid{\#bdb4b79}\footnote{\url{https://github.com/orbkit/orbkit/commit/bdb4b79669b4805249a7b1ade4c962157284f2fc}} 
\href{https://github.com/orbkit/orbkit/commit/bdb4b79669b4805249a7b1ade4c962157284f2fc}{{\texttt{\#bdb4b79}}} is an example of this kind,
% An example is the commit with \hashid{\#bdb4b79}\footnote{\url{https://github.com/orbkit/orbkit/commit/bdb4b79669b4805249a7b1ade4c962157284f2fc}}, 
which modified $45$ files 
by adding $1,336$ lines of code to the 
% with $1,336$ additional lines of code for the program 
% \texttt{orbkit/orbkit}\footnote{\url{https://github.com/orbkit/orbkit}} 
\href{https://github.com/orbkit/orbkit}{\texttt{orbkit/orbkit}}
(a Python-based program package for post-processing of wave function data from quantum chemical programs output files). 
We observed that later commits (\href{https://github.com/orbkit/orbkit/commit/a9d071a0c1261cf83ce986af1a68623ac58d143a}{{\texttt{\#a9d071a}}}
and 
\href{https://github.com/orbkit/orbkit/commit/8a97e8f794f66690622e34cd822b8a421c0a6fa8}{{\texttt{\#8a97e8f}}}) modified the files involved in this commit to fix incompatibility problems of Python 3 and problems about configuration settings.
%This commit was detected as fault-inducing because of fault-fix and refactoring changes that modified the files mainly related to Python3 compatibility and other program configuration settings. 
% The corresponding fault-fix commits such as 
% \hashid{\#a9d071a}\footnote{\url{https://github.com/orbkit/orbkit/commit/a9d071a0c1261cf83ce986af1a68623ac58d143a}}, 
%\href{https://github.com/orbkit/orbkit/commit/a9d071a0c1261cf83ce986af1a68623ac58d143a}{\hashid{\texttt{\#a9d071a}}}
%and 
% \hashid{\#8a97e8f}\footnote{\url{https://github.com/orbkit/orbkit/commit/8a97e8f794f66690622e34cd822b8a421c0a6fa8}} 
%\href{https://github.com/orbkit/orbkit/commit/8a97e8f794f66690622e34cd822b8a421c0a6fa8}{\hashid{\texttt{\#8a97e8f}}}
% include two more commits 
%are two other corresponding fault-fixing commits 
% that modified 
%modifying similar lines of codes.  

\nd Another example is the commit  
% \hashid{\#98e7c05}\footnote{\url{https://github.com/tmancal74/quantarhei/commit/98e7c058b375e191c4d8513dd880c18a537cb409}} 
\href{https://github.com/tmancal74/quantarhei/commit/98e7c058b375e191c4d8513dd880c18a537cb409}{{\texttt{\#98e7c05}}}
in the project \texttt{tmancal74/quantarhei} (a python-based simulator for molecular systems). The commit modified both the configuration files (`.yml') and the native Python code to integrate automatic detection of the file type and execution of its scripts. 
% Other quantum projects with similar problem
% % issues related to fault introduced during modification of configuration files 
% include 
In the following projects, we observed the same kind of faults: 
\texttt{m-labs/artiq}, 
% \texttt{rigetti/qvm}\footnote{\url{https://github.com/rigetti/qvm}} (a Simulator), 
\href{https://github.com/rigetti/qvm}{\texttt{rigetti/qvm}}
% \texttt{lneuhaus/pyrpl}\footnote{\url{https://github.com/lneuhaus/pyrpl}} 
\href{https://github.com/lneuhaus/pyrpl}{\texttt{lneuhaus/pyrpl}}
(Experimental), 
% \texttt{BBN-Q/Qlab}\footnote{\url{https://github.com/BBN-Q/Qlab}} 
\href{https://github.com/BBN-Q/Qlab}{\texttt{BBN-Q/Qlab}}
(Experimental) and 
% \texttt{XanaduAI/strawberryfields}\footnote{\url{https://github.com/XanaduAI/strawberryfields}} 
\href{https://github.com/XanaduAI/strawberryfields}{\texttt{XanaduAI/strawberryfields}}
(a quantum full stack library).

\begin{tcolorbox}
22 topics are extracted from the changes that introduced quantum software faults.
%representing the key areas commonly impacted by fault-inducing commits during quantum software development. 
%The topics cover the areas such as quality checks, test implementation, optimization procedures, code refactoring, release engineering process, environment, file management, and quantum/molecular mechanics.
Most of the topics can also be found in traditional software. Quantum developers can refer to the existing quality assurance approaches and practices in traditional software to mitigate faults in their programs. Future works need to study how to mitigate or avoid quantum-specific faults, such as those are related to quantum mechanics.
\end{tcolorbox}


\begin{figure}[ht]
%\scalebox{0.70}{
\center
\includegraphics[width=\linewidth]{image/boxplot_dist-edited.pdf}
\caption{Distributions of fault-inducing commits in each topic, which are sorted by the median number of the fault-inducing commits.}%For example, among $69\%$  of the projects (column `\% coverage' in Table \ref{tab:topics}) in `Configuration Files'  topic, the majority of the projects contributed about $15$ fault-inducing commit messages to the topic. [Le: The last sentence is not understandable]\Mehdi{I also can not understand the concept of this sentence!}} 
\label{fig:boxplot}
%}
\end{figure}


% The box-plot in 
\fig\ref{fig:boxplot} shows the distributions of the fault-inducing commits in 
% all the $22$ 
different topics (listed in Table \ref{tab:topics}). 
%We sorted the median number of the inducing commits for the projects in the Topic\mehdi{It is also explained in the caption of figure. I think we should not repeat it.}.  
We observed that there is a uniform distribution of the fault-inducing commits between the topics with the most dominating fault-inducing commits and the least dominating topic. In general, we can see that most of the fault-inducing commits are in the `Configuration Files' and `Dependency Management' topics (most dominating) whereas the topic `Path Integral' contains the least number of fault-inducing commits (least dominating). 



`Dependency Management' is a topic in release engineering~\cite{modern-release-bram,Openja:2020} about the different mechanisms to consolidate and centralize the dependencies information used by the projects such as the modules, dependency versions, maintaining reproducible builds, and library versions. According to Table \ref{tab:topics}, the faults related to `Dependency Management' is common to $73\%$ of the studied projects. An example of the fault-inducing commits is the commit \href{https://github.com/Qiskit/qiskit-aer/commit/c6f2013fcf1e958a716a1e3c0ed6481b207a5941}{{\texttt{\#c6f2013}}} in project
% \texttt{Qiskit/qiskit-aer}\footnote{\url{https://github.com/Qiskit/qiskit-aer}} 
\href{https://github.com/Qiskit/qiskit-aer}{\texttt{Qiskit/qiskit-aer}}.
%with
% \hashid{\#c6f2013}\footnote{\url{https://github.com/Qiskit/qiskit-aer/commit/c6f2013fcf1e958a716a1e3c0ed6481b207a5941}} 
%\href{https://github.com/Qiskit/qiskit-aer/commit/c6f2013fcf1e958a716a1e3c0ed6481b207a5941}{\hashid{\texttt{\#c6f2013}}}
The commit modified $10$ files with $313$ lines of code added and $292$ lines removed. These changes are related to the build system. We found a total of $66$ fault-inducing commits (about 6\% of all commits) in \texttt{Qiskit/qiskit-aer}, which are related to `Dependency Management'. 
We observed the similar faults from other quantum project:
% \href{}{\texttt{}}
% \texttt{quantumlib/Cirq}\footnote{\url{https://github.com/quantumlib/Cirq}}, 
\href{https://github.com/quantumlib/Cirq}{\texttt{quantumlib/Cirq}},
% \texttt{QE-Lab/OpenQL}\footnote{\url{https://github.com/QE-Lab/OpenQL}}, 
\href{https://github.com/QE-Lab/OpenQL}{\texttt{QE-Lab/OpenQL}},
% \texttt{Qiskit/qiskit-ignis}\footnote{\url{https://github.com/Qiskit/qiskit-ignis}}, 
\href{https://github.com/Qiskit/qiskit-ignis}{\texttt{Qiskit/qiskit-ignis}},
% \texttt{TRIQS/triqs}\footnote{\url{https://github.com/TRIQS/triqs}}, 
\href{https://github.com/TRIQS/triqs}{\texttt{TRIQS/triqs}},
and 
% \texttt{cp2k/cp2k}\footnote{\url{https://github.com/cp2k/cp2k}}.
\href{https://github.com/cp2k/cp2k}{\texttt{cp2k/cp2k}}.

In traditional software development, `Configuration Files' and `Dependency Management' are two kinds of activities that are subject to fault introduction. From Figure \ref{fig:boxplot}, we observed the same result in quantum software, which suggest that quantum developers should carefully manage their configuration files and dependencies. They can use tools or linters to avoid this kind of faults.
%Yet, they still find it challenging to manage project dependencies and implementation related to project's configuration files. 
%Hence maybe the reason for highly dominating with faulty commits among other topics\mehdi{not clear!!!}.


%\Le{General comments: along with the test related faults, we need to very carefully discuss the documentation related ``faults'', because they do not affect users and they do not affect software's behaviour. Two possible solutions: either we remove the discussion and data about test and documentation, or we very carefully define what a fault is and why we include test and documentation related ``faults''.}
%\nd Our analysis also identified documentation related topic as one of the major area modified when committing fault-inducing commits. We found that most (if not all) of the developers' changes are accompanied by reasonable documentation by manual analysis. The documentation related faults majorly fall under the category `Updates to the ReadMe' (the descriptions of the projects and its main-features accessible directly in the project repository), `in-code (source code) comments/ docstrings,' `changelog' (updates description and fault-fixes in the new release), `or other forms of documents or tutorials to guide the new users'. Also, we observed that some of these commits were detected as fault-inducing because they were associated with other files containing the real implementation. For example the commit \hashid{\#c2d27cc}\footnote{\url{https://github.com/PennyLaneAI/pennylane/commit/c2d27ccc005e46bba584b3f6a18fb9eed4824f88}} updated $55$ different files with $1,694$ added lines of code and $957$ lines removed including fault-fixes, refactoring different files whereby all the changes where documented within the `changelog.md' file. These kind of changes were across most of the commits made on the $75\%$ of the studied projects (according to \fig\ref{fig:boxplot}), including  \texttt{PennyLaneAI/pennylane}\footnote{\url{https://github.com/PennyLaneAI/pennylane}}, \texttt{catho/quantum}\footnote{\url{https://github.com/catho/quantum}}, \texttt{Qiskit/qiskit-terra} \footnote{\url{https://github.com/Qiskit/qiskit-terra}}, \texttt{rigetti/pyquil}\footnote{\url{https://github.com/rigetti/pyquil}}, and  \texttt{quantumlib/Cirq} \footnote{\url{https://github.com/quantumlib/Cirq}}.

\nd As shown in \fig\ref{fig:boxplot}, other topics that could be interesting to investigate due to the higher dominating fault-inducing commits include `Compiler Optimization',  `Calibration \& Visualization', `Program Optimization', `Data Structure \& Operations', `Gates Decomposition', and `Continuous Integration'. 


\begin{tcolorbox}
Most of the fault-inducing commits are in the topics `Configuration Files' and `Dependency Management' (most dominating topics) whereas the topic `Path Integral' contains the least number of fault-inducing commit (least dominating).
\end{tcolorbox}

%\input{image/charts/plot_commits}

\begin{figure}[ht]
%\scalebox{0.70}{
\center
\includegraphics[width=\linewidth]{image/boxplot_efforts-v2-edited.pdf}
\caption{The average time (in hours) between the fault-fixes and fault-inducing commits in the target quantum projects.}
\label{fig:bugs_effort}
%}
\end{figure}

We further examined %the time between fault introductions and fault fixes.
%date of fault-inducing commits and the fault-fixing ones for each topic. 
%We defined 
the time difference between the fault-inducing commits and the corresponding fault-fixing commits. We calculated the median of the time differences in a project as the life of the faults in the project.

\fig\ref{fig:bugs_effort} shows how long the faults lived in projects along the 22 topics.
%the time in which the faults introduced in the target projects remained life in each of the $22$ identified topics. 
We observed that the faults related to the topic `Chemical Calculation' remained for the longest time compared to other topics. `Chemical Calculation' is a topic in quantum-chemistry about applying mathematical calculations to investigate the electronic structure and molecular dynamics by employing the Schr{\"o}dinger method~\cite{berezin2012schrodinger}. This topic also captures different aspects of Atomic orbital, molecular orbital calculations, and their energies. A long life time of the faults in this topic
%The higher period the software faults related to `Chemical Calculation' remains life may 
implies that quantum developers took a lot of time to discover the software faults due to the insufficient debugging tools. It also implies the difficulties of implementing the necessary mathematical concepts when examining the chemical structures. One example of the changes that introduced such long life faults is the commit \path{#54b4c38} in the project \texttt{orbkit/orbkit}. 



==> subsections/droped-4.9.tex <==

\subsection{Preprocessing the Messages of Fault-Inducing Commits}\label{sub:preprocess}

%In this phase, we prepare our $133,654$ fault-inducing commit messages extracted in section \ref{sub:bug-inducing} 
We prepared fault-inducing commit messages extracted from the previous section for analyzing the topics involved in the messages.
% \mehdi{for classifying bug-inducing commit messages?!?!}. 
We first removed non-formatted texts or code snippets in the commit messages using regular expressions.
%The commit messages may include non formatted texts or code snippets, which need to be removed using regular expressions.  
% Further 
Then, we removed auto generated text by GitHub such as \emph{`Fixed in PR \#744 ', `Addressed in \#930'}. 
% removed the auto generated related text by GitHub that we could easily identify such as \emph{`Fixed in PR \#744 ', `Addressed in \#930'}.
Next, we removed the text related to login or name of the developer starting with the character symbol `@', as well as the HTML links or email addresses. We also removed other possible special characters such as `\#', `//`, `>', `?', `\_', `:', `+`, `='.  
To further clean up the message texts, we used MALLET list-of-stopwords~\cite{mallet:stopwords}
% ~\footnote{\url{https://github.com/mengjunxie/ae-lda/blob/master/misc/mallet-stopwords-en.txt}} 
to identify and remove stopwords from the commit messages.
% We then used a list of stopwords to removed the words identify as stopword~\cite{Joshi:2012:Tostop-not} such as `the', `a', `for', `be', `is' among others, using .  
Finally, we reduced words to their stemmed representation using Porter stemmer~\cite{Porter01}. 
For example, words like `testing’, `tests' and `tested' are  reduced  to ‘test’; `configuration’, `configure’ and `configured’ are reduced to `configr’.
%\mehdi{can we use a bullet point list and mention all preprocessing items phases?}


\subsection{Modelling and Labelling the Fault-Inducing Commits}\label{sec:model-labels}

\MO{Reviewer1: -It is important to highlight what does it mean choosing K and I considering topics good granularity. What a good granularity is in this context?}

%\Le{I will read RQ4 first, then decide whether we need to keep this subsection.}
%\Le{We actually did manual classifications on the bugs, so we may not need to do topic modeling.}
In this section, we aim to extract information from preprocessed fault-inducing commit messages and model them as topics using clustering techniques.
% In this section, we aim to model and extract information using clustering techniques on the preprocessed fault-inducing messages from section \ref{sub:preprocess} into topics. 
We chose MALLET~\cite{MALLET}, a toolkit that uses Gibbs sampling algorithms~\cite{GibbsAlgorithm}, implementing Latent Dirichlet Allocation (LDA)~\cite{Blei:LDA:2003}. 
LDA is a widely used and state-of-the-art technique of topic modeling to represent a topic as a set of frequently co-occurring words in a corpus of text that approximate real-world situations~\cite{Mehdi:GoingBig:2019}. LDA categorizes the corpus into $K$ topics after $I$ grouping iterations. 
Also, LDA is probabilistic, where the topics are presented as a vector of word probabilities
and a document is considered as a vector of topic probabilities. 
Topic with the highest assigned proportional value is considered as dominant topic. 
% A topic is considered as the most dominant if the proportional value assigned is higher compared to others. 

% During the clustering, we choose both bi-grams and uni-gram topic lists \mehdi{}. 
We used both of bigram and unigram topic list in LDA. 
We used bigram to improve the quality of the text during clustering process as proven in the previous study by Tan~\cite{tan:2002:bigrams}. The number of topics ($K$) and the iteration groupings ($I$) are user defined parameters  to control the returned topics granularity~\cite{Anton:What-are-developers:2014}. Treude and Wagner~\cite{Treude:Predicting-Good-Configurations:2019} in their previous study noted that due to the different characteristics, some of the popular topic modelling parameter configuration rules of thumb may not be applicable to textual corpora from GitHub and StackOverflow.
% for a better model fit. 
% We therefore take this into consideration when setting the configuration parameters.
To discover the right number of topics for our dataset, 
firstly we carried out experiments with different values of $K$ and $I$ and chose the values giving us the topics of good granularity.
% we first experimented with different values of $K$ and $I$ and choose the values that gave us topics of good granularity. 
We did experiments using different values of K starting from $5$ to $60$ in the incremental range of  $5$, where as for $I$ iteration we vary our values from $500$ to $5,000$ in the range of $500$, following the previous studies that uses GitHub dataset~\cite{Linstead:GNOME-bug-report,Hindle:Automated-Topic:2011,Liao:Issue-Related:2018} or stackoverflow dataset~\cite{Mehdi:GoingBig:2019,Christoffer:Mobile-Developers:2016,Kartik:Web-Developers:2014,Syed:Concurrency:2018, Openja:2020} with LDA topic modelling technique. 
LDA using 
% In our experiment using the values 
$K=25$ and $I=3,000$ gave us a better meaning, as well as captured the broader range of topics in quantum computing within our dataset.

The next step was manually labelling all the $25$ returned topics categories (i.e., the output of running MALLET). First, the output documents were shared among the labelling team (the first and second authors). Each document in a group contains the top $30$ keywords extracted from common, occurring words and the documents' corresponding probabilistic value scores. 
Intuitively, a document with a higher probability value has a higher contribution to that topic and impacts the topic's label favorably.
% compared to the rest. 
Hence, we use the dominant probability to sort documents in descending order
% from highest to lowest 
and assign the right topic name. 
We randomly read through at least the top $15$ to $20$ documents in each group and the top $30$ keywords to assign a topic name to each group. During the labelling, the authors reached a common agreement before assigning each topic name.

The authors also identified three topics related to the documentation, docstrings/ general comments, and test implementation during the topic labelling. Manual investigation revealed that these topics were not directly related to fault-inducing commits, but they were submitted together with changes that induce faults. 
% For example, we found that most of commits submitted 
For example, we found that most of the mentioned commits include further updates to the documentation related files such as changelog, Readme, and docstring/comments such as the commit
% \texttt{\#c2d27cc}.
\href{https://github.com/PennyLaneAI/pennylane/commit/c2d27ccc005e46bba584b3f6a18fb9eed4824f88}{{\texttt{\#c2d27cc}}} in \path{PennyLaneAI/pennylane}. 
These kind of changes were identified in many other projects such as \path{catho/quantum}, \path{Qiskit/qiskit-terra}, \path{rigetti/pyquil}, and  \path{quantumlib/Cirq}. 
The authors therefore agreed and removed these three topics from the list of the $25$ groups.  

Our final list has a total of $22$ topics shown in Table \ref{tab:topics}. The analysis of this step answers our \textbf{RQ4} and will be discussed in Section \ref{sec:result-bugs-introduced}.




==> subsections/intro-comments.tex <==

\MO{Reviewer1: Minor to Address
-------------
\begin{itemize}
    \item In presenting the results for RQ1 you mention both quantum and non-quantum software but from my understanding you only looked at quantum systems while non-quantum results are derived from previous literature. Please clarify this in the paper. \BLUE{corrected this, by removing the non-quantum in RQ1 intro.}
     \item  In the Introduction while presenting RQ1 it would be better to anticipate the usage of SonarQube instead of simply referring to it as [29].
     \item   I would remove the paragraph before the paper structure in the Introduction since we do not have enough elements there to understand what is being reported, whereas referring to best practices for quantum software developers are there reported somewhere in the paper? Are those an outcome of the paper? It seems no, I would suggest moving that statement somewhere as future direction for the study being reported here. \BLUE{removed}
    \item Missed reference at page 4. [37 ?, 39 ...]. Please fix it. \BLUE{fixed}
    \item Use an ordering for multiple references. As an example, [19, 26, 12, 13, 27] becomes [12, 13, 19, 26,27]. \BLUE{Not fixed for all, Mona can you help to order the citation?}
    \item  The detailed description of [55] in section 3.1 is unneeded. Think about removing it.
   \item  Figure 1 has to be fixed since you are referring to wrong section identifiers. Section 5 reports the results while Section 4 describes the whole methodology. \BLUE{fixed}
   \item  Missed reference to QoSE at page 7.
   \item  The statement TDs with major and critical severity require most effort to fix do not hold on the whole categories if you look at Table 4b.
\end{itemize}
Typos
--------------------
\begin{itemize}
    \item I would suggest a proof-reading of the paper since there were many typos that need to be addressed. In the following I will report only some of them.
    \item Page 3: was introduce -> was introduced
    \item Page 4: they represented that -> they reported that. I found that very often you replace report with represent.
    \item Page 5: that is resulted from -> due to
    \item Page 9: box-plot corresponds to 30 -> box-plot corresponding to 30
    \item Page 13: assigned proportional -> assigned probability
\end{itemize}}


\MO{Reviewer2: 2. There are places in the paper where a term/idea is introduced, without further details, and sometimes is only supported with an external reference. Some examples:
        - Section 1, RQ1: it's mentioned: "technical debts [...] represented as code smells and coding error [...]", but there are no further details on the definition of "technical debt", or comparison between the definition of "code smells" and "code errors".
        - on the same paragraph: "belongs to *major category*". The reader with little knowledge on severity levels of SonarQube will have no idea until Table 2 (page 10), what "major category" refers to.
        - Section 1, RQ4: In the second paragraph, multiple commit topics (from Table 10) are mentioned which are not meaningful to the reader without definitions. Moreover, at the end you say "these 10 activities", but you mentioned 13 activities beforehand.
3. The captions of some tables are not aligned center. Table 1 and 3, for instance, are aligned left.
4. Table 4:
        - The subscription for tables 4a and 4b is too small to read.
        - The numbers are not aligned and are hard to compare. It would be nice to have all decimal points aligned vertically.
        # Minor questions/issues:
\begin{itemize}
    \item  Section 1, line 5: "for checking and correcting errors". Which errors?
    \item  Section 1, line 5,6: It would be nicer if you could add references for "examples of operational quantum software".
   \item Section 1, RQ3: Wrong citation for "and their types [32]". The link simply refers to the homepage of the latest SonarQube official documentation, but not any "type".
   \item  Section 1, RQ1, RQ3: "code convention" vs. "convention". Please use the full name for the sake of consistency.
   \item  Section 3.2: While the term "technical debts" is used all over the paper, this paragraph looks like an exception by using the shortened form ("TD").
   \item  Section 3.2: "comparison of 9 TD tools" -> "comparison of 9 technical debts identifier tools"
\end{itemize}
# Verifiability (ability to replicate)
Although the paper describes all the steps clearly, the level of detail provided is not sufficient to replicate the process. This is mainly due to two reasons:
The required information is missing (e.g., the API call used in step 4.1, or the list of 22 topics obtained in the last step).
The information is referenced as an external work (e.g., "To identify the fault-fixing commits, we used a list of keywords suggested in previous studies [..]").
I highly recommend presenting all the information required to reconduct the study in form of a replication package and make the paper self-contained.
# Suggestions
- In step 4.1, you filter repositories based on the number of forks they have in a separate step after using GitHub API call. However, this could be integrated into the same GitHub API search call. See: https://docs.github.com/en/github/searching-for-information-on-github/searching-on-github/searching-for-repositories#search-by-number-of-forks
# Typos
\begin{itemize}
    \item Section 2.2: "we refer our readers to [37?": Missing citation? \BLUE{fixed}
    \item Section 3.1: "seven different type of" -> "seven different types of" \BLUE{fixed}
    \item  Section 3.3: "On the one hand, the proved" -> "On the one hand, they proved" \BLUE{section removed}
   \item Section 4.1: "\_" -> "\_" \BLUE{fixed}
   \item  Section 5.4: Inconsistency in capitalization: "Code Integration" vs. "Chemical calculation" \BLUE{To be fixed by removing the whole section}
\end{itemize}}


==> subsections/regression_model_old_dataset_tbl.tex <==
\begin{table}
    \caption{$p$-values for statistical significance and the coefficient for the MLR model based on individual quantum categories. The model uses the number of fault-inducing commits as dependent variable and the list of independent variables derived from technical debts types. \\ Statistical significance denoted as: $***< 0.001,  ** < 0.01, * < 0.05 $,\\ $\dag$ variable removed during VIF analysis,\\ $\ddag$ variable removed during stepwise criteria.
    } 
    \label{tab:tbl_tags_corr_debt_qt_category}
	\centering
	\begin{adjustbox}{width=\columnwidth,center}
	\small
        \begin{tabular}{l| c c c c c c c c c c}\toprule
        \rowcolor{gray!20}
        \textbf{coef/p-value}  & \textbf{Fstack}&  \textbf{Tkit}&   \textbf{Exp}&  \textbf{Sim}&  \textbf{Crypt}&   \textbf{Comp}& \textbf{Alg}& \textbf{Chem}&   \textbf{Ass}&\textbf{Ann}\\ \midrule
        is\_smelly&\hlcyan{7.6910$^{***}$}&\hlcyan{5.3580$^{***}$}&\hlcyan{0.0642$^{***}$}&\hlcyan{9.3227$^{***}$}&\hlcyan{256.0$^{***}$}&\hlcyan{4.4$^{***}$}&\hlcyan{0.1613$^{***}$}&\hlcyan{12.4$^{***}$}&\hlcyan{0.0003$^{***}$}&\hlcyan{8.0$^{***}$}\\ %hline
        is\_erroneous&\hlcyan{5.2814$^{***}$}&\hlcyan{4.1233$^{***}$}&\hlcyan{0.0451$^{**}$}&$\dag$&$\dag$&$\dag$&\hlcyan{0.2072$^{***}$}&\hlcyan{7.3$^{*}$}&\hlcyan{8.533e-05$^{*}$}&$\dag$\\ \midrule
        accessibility&$\dag$&\hlcyan{2.3$^{***}$}&$\ddag$&$\dag$&\hlcyan{294.7$^{***}$}&$\dag$&$\dag$&\hlcyan{17.0$^{*}$}&$\dag$&$\dag$\\
        brain-overload&\hlcyan{1.3299$^{***}$}&\hlcyan{1.43$^{***}$}&\hlcyan{0.0169$^{***}$}&\hlcyan{1.53$^{***}$}&$\dag$&\hlcyan{0.7913$^{***}$}&\hlcyan{0.9041$^{***}$}&\hlcyan{3.92$^{***}$}&\hlcyan{1.165e-05$^{*}$}&\hlcyan{2.8e+04$^{***}$}\\
        design&$\ddag$&$\dag$&$\dag$&$\ddag$&$\dag$&$\dag$&\hlcyan{4.0313$^{***}$}&$\dag$&$\dag$&$\dag$\\
        unused&$\ddag$&\hlcyan{0.569$^{***}$}&$\dag$&$\dag$&$\dag$&\hlcyan{0.533$^{**}$}&$\dag$&$\dag$&$\ddag$&$\dag$\\
        convention&\hlcyan{0.097$^{***}$}&$\dag$&$\dag$&$\dag$&$\dag$&$\dag$&\hlcyan{0.380$^{***}$}&$\dag$&$\dag$&$\dag$\\
        cwe&$\ddag$&\hlcyan{4.821$^{***}$}&$\dag$&$\dag$&$\dag$&$\ddag$&$\dag$&$\dag$&$\dag$&$\dag$\\
        redundant&$\dag$&$\ddag$&$\dag$&$\dag$&$\dag$&$\dag$&\hlcyan{0.52$^{***}$}&$\dag$&$\dag$&$\dag$\\
        confusing&$\ddag$&$\dag$&\hlcyan{236.1$^{***}$}&$\dag$&$\dag$&$\dag$&\hlcyan{0.028$^{***}$}&$\dag$&$\dag$&$\ddag$\\
        error-handling&$\dag$&$\dag$&\hlcyan{27.98$^{***}$}&$\ddag$&$\dag$&\hlcyan{8.03$^{***}$}&$\dag$&$\dag$&\hlcyan{0.0002$^{**}$}&\hlcyan{22.52$^{***}$}\\
        obsolete&$\dag$&\hlcyan{40.20$^{***}$}&$\dag$&$\dag$&$\dag$&$\dag$&\hlcyan{46.60$^{***}$}&$\dag$&$\dag$&$\dag$\\
        user-experience&$\dag$&$\dag$&$\dag$&$\dag$&\hlcyan{256.0$^{***}$}&$\dag$&\hlcyan{80.64$^{**}$}&\hlcyan{210.45$^{***}$}&$\dag$&$\dag$\\
        suspicious&\hlcyan{0.549$^{***}$}&\hlcyan{1.675$^{***}$}&$\dag$&$\dag$&$\ddag$&$\ddag$&\hlcyan{0.0113$^{*}$}&$\dag$&\hlcyan{6.4e-05$^{***}$}&$\dag$\\ %hline
        \bottomrule
        Adj. $R^{2}$&\multicolumn{1}{r}{0.062}&\multicolumn{1}{r}{0.125}&\multicolumn{1}{r}{0.093}&\multicolumn{1}{r}{0.004}&\multicolumn{1}{r}{0.488}&\multicolumn{1}{r}{0.007}&\multicolumn{1}{r}{0.189}&\multicolumn{1}{r}{0.010}&\multicolumn{1}{r}{0.365}&\multicolumn{1}{r}{0.174}\\ %hline
        Prob (F-stat)&\multicolumn{1}{r}{1.37e-133}&\multicolumn{1}{r}{0.00}&\multicolumn{1}{r}{2.85e-84}&\multicolumn{1}{r}{5.21e-13}&\multicolumn{1}{r}{0.00}&\multicolumn{1}{r}{4.75e-23}&\multicolumn{1}{r}{2.60e-316}&\multicolumn{1}{r}{1.43e-121}&\multicolumn{1}{r}{7.94e-121}&\multicolumn{1}{r}{2.15e-54}\\ %hline
        AIC:&\multicolumn{1}{r}{8.071e+04}&\multicolumn{1}{r}{1.285e+05}&\multicolumn{1}{r}{-738.4}&\multicolumn{1}{r}{1.419e+05}&\multicolumn{1}{r}{3.896e+04}&\multicolumn{1}{r}{1.145e+05}&\multicolumn{1}{r}{3444.}&\multicolumn{1}{r}{6.272e+05}&\multicolumn{1}{r}{-1.651e+04}&\multicolumn{1}{r}{1.115e+04}\\ %hline
        \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table}

==> tables/tbl_efforts.tex <==
\begin{table}
\caption{Effort required to fix technical debts in terms of debt types and severity types.}
%\caption{Distribution of the required effort (the time in minutes) to fix issues in a category. 
%\mehdi{I think we can move the description highlighted with red to the text, not in the caption of table.} \textcolor{red}{We analyzed the effort both on the issue types (\emph{SQ-Bug} or \emph{Code Smell}) and their severity(\emph{critical, major, blocker, or minor}).  We report the mean percentage values across the projects in a category.  $\sigma$ denotes the standard deviation of the percentage values across the projects in a category.} } 
\label{tab:issue-types}

	\centering
	\scalebox{0.65}{
	\begin{subtable}[t]{4in}
		\caption{Effort required to fix technical debts in terms of the debt types (coding errors and code smells)}	
		\label{subtab:effort_type}
		\centering
        \begin{tabular}{l| r r }\toprule
            \textbf{Category}  & \textbf{\%Error($\sigma$)} & \textbf{\%Smell($\sigma$)}\\ \midrule
            Experimentation&29.52 (6.01)&70.48 (6.2)\\ %hline
            Toolkit&24.47(6.82) & 75.53 (16.87)\\ %hline
            Quantum Annealing&30.66 (5.39)&69.34 (5.21)\\ %hline
            Assembly&21.68 (5.51)&78.32 (10.36)\\ %hline
            %Fun/ Game&43.09(3.03)&56.91(9.69)\\ %hline
            Compiler&1.82 (2.35)&98.18 (9.77)\\ %hline
            Cryptography&1.36 (3.01)&98.64 (9.12)\\ %hline
            Full-stack Library&8.37 (3.76)&91.63 (18.91)\\ %hline
            Simulator&5.66 (4.64)&94.34 (5.63)\\ %hline
            Quantum-Chemistry&4.56 (5.86)&95.44 (25.41)\\ %hline
            Quantum Algorithsm&12.27 (5.61)&87.73 (10.01)\\ %hline
            \bottomrule
            \rowcolor{gray!15}
            \textbf{Total Mean}& \textbf{14.04 (4.90)}&	\textbf{85.96 (11.75)}\\ %\hline&	\textbf{0.03(2.1)}\\ %\hline
            \bottomrule
        \end{tabular}  
	\end{subtable}
	
	\hspace{2cm}
	
	\begin{subtable}[t]{4in}
		\caption{Effort required to fix the technical debts in terms of severity}\label{subtab:effort_severity}
		\centering		
		\begin{adjustbox}{center}
         	\begin{tabular}{l |r r r r}\toprule
                \textbf{Category} & \textbf{\%critical($\sigma$)} & \textbf{\%major($\sigma$)}& \textbf{\%minor($\sigma$)} &\textbf{\%blocker($\sigma$)} \\ \midrule
                Experimentation&14.45 (12.4)&30.57 (5.5)&32.28 (1.2)&22.71 (2.1) \\ %hline
                Toolkit&33.91 (39.7)&28.29 (6.4)&14.37 (1.4)&23.43 (2.5) \\ %hline
                Quantum Annealing&23.9 (8.5)&40.84 (5.9)&18.51 (1.4)&16.74 (2.1) \\ %hline
                Assembly&44.13 (24.1)&29.85 (5.8)&14.18 (1.3)&11.83 (1) \\ %hline
                %Fun/ Game&7(66.6)&55.28(7.4)&25.36(1.2)&12.36(3.8) \\ %hline
                Compiler&80.84 (31)&15.72 (5)&2.24 (1.5)&1.2 (7.1) \\ %hline
                Cryptography&26.7 (16.3)&64.89 (8)&8.01 (1.6)&0.39 (2.2) \\ %hline
                Full-stack Library&52.95 (37)&31.36 (5.3)&8.58 (1.5)&7.11 (0.9) \\ %hline
                Simulator&31.12 (15.7)&52.38 (4.2)&14.48 (1.4)&2.03 (1.7) \\ %hline
                Quantum-Chemistry&37.03 (58.8)&42.19 (5.7)&16.42 (1.2)&4.36 (3.5) \\ %hline
                Quantum Algorithsm&13.77 (20.3)&66.98 (5.5)&7.62 (1.4)&11.63 (2.2) \\ %hline
                \bottomrule
    			\rowcolor{gray!15}
    			\textbf{Total Mean}& \textbf{35.88 (26.4)}&\textbf{40.31 (5.7)}&\textbf{13.67 (1.4)}&\textbf{10.14 (2.5)}\\  %\hline
    			\bottomrule
    		\end{tabular}  
		\end{adjustbox}	
	\end{subtable}
	}
\end{table}
